Multi-Task Learning as Multi-Objective Optimization

In multi-task learning, multiple tasks are solved jointly, sharing inductive bias between them. Multi-task learning is inherently a multi-objective problem because different tasks may conflict, necessitating a trade-off. A common compromise is to optimize a proxy objective that minimizes a weighted linear combination of per-task losses. However, this workaround is only valid when the tasks do not compete, which is rarely the case. In this paper, we explicitly cast multi-task learning as multi-objective optimization, with the overall objective of finding a Pareto optimal solution. To this end, we use algorithms developed in the gradient-based multi-objective optimization literature. These algorithms are not directly applicable to large-scale learning problems since they scale poorly with the dimensionality of the gradients and the number of tasks. We therefore propose an upper bound for the multi-objective loss and show that it can be optimized efficiently. We further prove that optimizing this upper bound yields a Pareto optimal solution under realistic assumptions. We apply our method to a variety of multi-task deep learning problems including digit classification, scene understanding (joint semantic segmentation, instance segmentation, and depth estimation), and multi-label classification. Our method produces higher-performing models than recent multi-task learning formulations or per-task training.

==> tex/exp_multi_label_figure.tex <==
\begin{tabular}[t]{@{}c@{\hspace{4mm}}r@{}}
\begin{minipage}{0.67\textwidth}
%\vspace{-9mm}
\begin{tabular}{@{}c@{}c@{}}
\includegraphics[width=\textwidth]{radar_full_new}
\end{tabular}
%\vspace{-5mm}
\captionof{figure}{Radar charts of percentage error per attribute on CelebA \citep{celeba}. Lower is better. We divide attributes into two sets for legibility: easy on the left, hard on the right. Zoom in for details.}
\label{fig:multi_label_radar}
\vspace{5mm}
\end{minipage}&
\begin{minipage}{0.3\textwidth}
\vspace{-5mm}
\captionof{table}{Mean error of MTL algorithms in multi-label classification on CelebA \citep{celeba}. Percentage error of each attribute is computed separately and then averaged. Lower is better.}
\begin{tabular}{r@{\hspace{2mm}}c@{}}
\toprule
& Average  \\
&  error \\
\midrule
Single task & $8.77$ \\
Uniform scaling & $9.62$ \\
\citealt{Kendall2018} & $9.53$ \\
GradNorm & $8.44$ \\
Ours & $\mathbf{8.25}$  \\
\bottomrule
\end{tabular}
\label{table:multi_label_bar}
\end{minipage}
\vspace{-5mm}
\end{tabular}

